Online Spatiotemporal Action Detection and Prediction via Causal Representations

In this thesis, we focus on video action understanding problems from an online and real-time processing point of view. We start with the conversion of the traditional offline spatiotemporal action detection pipeline into an online spatiotemporal action tube detection system. An action tube is a set of bounding connected over time, which bounds an action instance in space and time. Next, we explore the future prediction capabilities of such detection methods by extending an existing action tube into the future by regression. Later, we seek to establish that online/causal representations can achieve similar performance to that of offline three dimensional (3D) convolutional neural networks (CNNs) on various tasks, including action recognition, temporal action segmentation and early prediction.

==> pads/epiface.tex <==
\newpage
\begin{center}	
{\large
\textbf{Epiface}
}
\end{center}
\addcontentsline{toc}{chapter}{Epiface}    
\vspace{1cm}
``It does not always end the way we wish it had.''

I would like to start the end by saying thank you to the readers. You got so far and I hope along the way you enjoyed and learned few new things.

Now, in this thesis we have extensivly discussed and proposed solutions for spatiotemopral action detection problem. Towards the end we also learned about prediction and causal representations.

==> pads/titlepage.tex <==
\begin{titlepage}

	\begin{minipage}{0.9\textwidth}
	%\vspace{2cm}
	\end{minipage}
	
	\begin{center}
		\Large
		\textbf{ONLINE SPATIOTEMPORAL ACTION DETECTION AND PREDICTION VIA CAUSAL REPRESENTATIONS} 
		%Towards Casual Action Tube Prediction}
	\end{center}	
		
	\vspace{2.5cm}
		
		
	\begin{center}		
		\Large
		{GURKIRT SINGH}
	\end{center}
	
	\vspace{0.5in}
	
	\begin{center}
	Ph.D.
\end{center}
% 		%\Large
%             A Thesis Submitted in Partial Fulfilment\\
%             of the Requirements for the Degree of \\
%             Doctor of Philosophy    \\
%             in \\
% 	Computer Science and Mathematics
% 	\end{center}
	
	
	
% 	\vspace{0.3in}

% 	\begin{center}
% 	%Department of Computing and Communication Technologies\\
% 	Visual Artificial Intelligence Lab\\
% 	School of Engineering, Computing and Mathematics\\
% 	Oxford Brookes University
% 	\end{center}
	
	\vspace{0.5in}

	
% 	\begin{center}
% 	Supervised by :\\
% 	Prof. Fabio Cuzzolin and Prof. Nigel Crook \\
% % 		 \footnotesize           
% % 		A dissertation submitted to the Faculty of Technology in partial fulfilment \\
% % 		of the requirements of the award of Doctor of Philosophy.  
% 	\end{center}

% 	\vspace{0.1in}
	
	\begin{center}		
		\small
		2019
	\end{center}
	
\end{titlepage}

